Manifold Path Guiding for Importance Sampling Specular Chains

Complex visual effects such as caustics are often produced by light paths containing multiple consecutive specular vertices (dubbed specular chains), which pose a challenge to unbiased estimation in Monte Carlo rendering. In this work, we study the light transport behavior within a sub-path that is comprised of a specular chain and two non-specular separators. We show that the specular manifolds formed by all the sub-paths could be exploited to provide coherence among sub-paths. By reconstructing continuous energy distributions from historical and coherent sub-paths, seed chains can be generated in the context of importance sampling and converge to admissible chains through manifold walks. We verify that importance sampling the seed chain in the continuous space reaches the goal of importance sampling the discrete admissible specular chain. Based on these observations and theoretical analyses, a progressive pipeline, manifold path guiding, is designed and implemented to importance sample challenging paths featuring long specular chains. To our best knowledge, this is the first general framework for importance sampling discrete specular chains in regular Monte Carlo rendering. Extensive experiments demonstrate that our method outperforms state-of-the-art unbiased solutions with up to 40x variance reduction, especially in typical scenes containing long specular chains and complex visibility.

==> 6-results.tex <==

\begin{figure*}[htbp]
\centering
	\begin{minipage}{1.00\linewidth}
  			\includegraphics[width=1.0\linewidth]{imgs/result/lamp.pdf}
	\end{minipage}
	\begin{minipage}{1.00\linewidth}
  			\includegraphics[width=1.0\linewidth]{imgs/result/flower.pdf}
	\end{minipage}
	\begin{minipage}{1.00\linewidth}
  			\includegraphics[width=1.0\linewidth]{imgs/result/slabs.pdf} % finalized
	\end{minipage}
  \caption{\textbf{Equal-time comparison\ff{s}} among Path Tracing (PT), the improved Practical Path Guiding (PPG) \cite{Muller17, mueller19guiding}, Variance-Aware Path Guiding (VAPG) \cite{Rath2020VarianceawarePG}, parallax-aware VMM Path Guiding (VMMPG) \cite{Ruppert2020RobustFO}, the original Specular Manifold Sampling (SMS) \cite{Zeltner20}, a modified version of SMS (SMS*) and our method on three scenes. 
  }
  \Description{...}
  \label{fig_result_2}
\end{figure*}

\section{Results}








We have implemented our approach in the Mitsuba 2 Renderer \cite{Mitsuba2} as a new integrator. 
In this section, we will describe our experimental setup, compare our approach to related methods, and validate our building blocks.

All our test scenes have been rendered on a compute node with 32 2.50 GHz cores of Xeon E5-2682 v4 processors. Since we focus on high-frequency light transport, we only use artificial point and small area light sources to cast caustics and handle them using the proposed approach. Other light transport portions involving environmental lighting are handled by conventional path tracing. We set the max length of paths to 15. Russian roulette starts from bounce 5 with probability $\gamma = 0.95$. Unless otherwise mentioned, we do \emph{not} enable product importance sampling or selective activation for a more fair comparison with related methods.

The reference images of \textsc{Lamp}, \textsc{Flower}, and \textsc{Double Slabs} are generated using path tracing, whereas the others are rendered with our modified SMS at high sample rates. \ff{Some of our results report the number of samples per pixel in the form of ``$n+m$'', meaning $n$ spp for training and $m$ spp for rendering.}

\subsection{Comparisons with previous approaches}

\paragraph{Comparison with unbiased MC approaches}

In Fig. \ref{fig_result_2}, we show the equal-time comparison of our approach against PT, PPG \cite{mueller19guiding}, VAPG \cite{Rath2020VarianceawarePG}, VMMPG \cite{Ruppert2020RobustFO}, the original SMS \cite{Zeltner20}, and our modified SMS on three scenes: \textsc{Lamp}, \textsc{Flower} and \textsc{Double Slabs}.

\begin{figure}[tbp]
\centering
	\begin{minipage}{1.00\linewidth}
  			\includegraphics[width=1.0\linewidth] {imgs/result/slab.pdf} % finalized
	\end{minipage}
  \caption{\textbf{Equal-time comparison} between the original SMS \cite{Zeltner20} and our method on the \textsc{Slab} scene. In order to validate the effect of directional sampling, we use a fixed chain length ($n=2$) and also neglect reflection on the dielectric surface. 
  }
  \Description{...}
  \label{fig_result_1}
\end{figure}  
\begin{figure}[tbp]
\centering
	\begin{minipage}{1.00\linewidth}
  			\includegraphics[width=0.5\linewidth]{imgs/result/convplot_slabs.pdf} % finalized
  			\includegraphics[width=0.5\linewidth]{imgs/result/convplot_lamp.pdf} % finalized
	\end{minipage}
\caption{\textbf{Convergence curves of two testing scenes.} 
We compare our method with PT, PPG, and SMS* on the evolution of MSE with respect to the total rendering (including training) time. The standard deviation of the MSE is shown as shaded regions.
} 
  \Description{...} 
  \label{fig_result_convergence}
\end{figure}
Conventional guiding approaches, such as PPG, rely on online learned distributions to perform path sampling. They generally work well but will encounter difficulties in dealing with glossy or specular interactions since the radiance distribution involves high-frequency variations. Visual comparisons clearly show that a typically guided path tracer, such as PPG, VAPG, and VMMPG, fails to handle challenging light paths involving specular vertices, leading to many outliers and energy loss. 

Although our approach also adopts reconstructed energy distributions as guidance, its usage is quite different. First, our distribution is reconstructed from admissible sub-path samples, which is beneficial for exploring high-frequency regions. Second, the reconstructed distribution is used to sample seed chains instead of light paths. Therefore, even inaccurate distributions can still work well. Consequently, our method succeeds in covering all challenging lighting effects with much fewer fireflies.

\begin{figure}[tbp]
\centering
  			\includegraphics[width=1\linewidth]{imgs/result/paper03b.pdf}
     
     \includegraphics[width=1\linewidth]{imgs/result/paper03b2.pdf}
  			
  \caption{
  \textbf{Equal-time (5 min) comparison} between MLT \cite{Veach97MLT}, MEMLT \cite{Jakob12} and our method.
  } 
  \Description{...}
  \label{fig_result_other}
\end{figure}



SMS is the state-of-the-art approach tailored for the unbiased simulation of specular light transport. The original SMS can only support a user-specified and fixed chain length. We extend it (denoted as SMS*) using our initialization (Section 5.4) to support various specular chain lengths and scattering types. 
Although this enables handling all types of specular chains, it has the risk of higher variance (see the \textsc{Lamp} scene) than the original SMS since the sample budget is amortized for various types of chains.

Thus, to further demonstrate the effect of our importance sampling strategy, we also choose a dominant type of chain for each scene ($RT$ for \textsc{Lamp}, $TTR$ for \textsc{Flower}, and $TTTT$ for \textsc{Double Slabs}) and present the results rendered by the original SMS in Fig. \ref{fig_result_2}. 
Even in this way, the original SMS still tends to produce noticeable noise since it samples seed chains uniformly.
This is particularly obvious in areas that correspond to admissible chains with extremely small convergence basins, e.g., the bottom of the slabs. 

Our method exploits progressively generated sub-path samples to reconstruct and refine continuous distributions for sampling seed chains, thus providing high-quality, unbiased rendering for challenging SDS paths. Even at relatively low sample rates, our method still outperforms its competitors with much lower variance. 


We further validate the benefit of our directional importance sampling in Fig. \ref{fig_result_1}, where we disable the sampling of chain length and type in our method and compare with the original SMS to validate the effect of directional importance sampling. 
As highlighted in the closeups, due to efficient importance sampling, our approach generates more samples and produces results with far less noise. 
A complete ablation study is shown in the supplemental document, which validates the effectiveness of length sampling, type sampling, and directional sampling, respectively.


In Fig. \ref{fig_result_convergence}, we evaluate the accuracy in terms of MSE with respect to the running time, showing the fast convergence provided by our method. Thanks to the energy-based sampling distribution, our method consistently outperforms previous ones as the running time increases and achieves a large margin at a high sampling rate.



\begin{figure}[tbp]
\centering
  			
  			\includegraphics[width=1.0\linewidth]{imgs/result/paper03c.pdf}
  \caption{
  \textbf{Equal-time (5 min) comparison} between SPPM \cite{Hachisuka09SPPM}, UPSMCMC \cite{Sik2016RobustLT}, and our method. 
  } 
  \Description{...}
  \label{fig_result_biased}
\end{figure}


\paragraph{Comparison with unbiased MCMC approaches} 

\begin{figure*}[tbp]
\centering
 
	\begin{minipage}{0.495\linewidth}
  		\includegraphics[width=1.0\linewidth]{imgs/result/paper08a_small_stone.pdf} 
	\end{minipage}
	\begin{minipage}{0.495\linewidth}
  		\includegraphics[width=1.0\linewidth]{imgs/result/paper08a_small_lamp.pdf} 
	\end{minipage}

 
  \caption{\textbf{Choices of building blocks.}
  \textbf{Left:}
  we perform equal-time comparisons of various spatial and directional structures. 
  \textbf{Right:}
  comparisons of different spatial filtering strategies.
  We report the full-image MSE, SPP, and the overhead of sampling. 
  More scenes are shown in the supplemental document.
  } 
  \Description{...}
  \label{fig_val_spatial}
\end{figure*}


\begin{figure*}[tbp]
\centering

	\begin{minipage}{0.33\linewidth}
  		\includegraphics[width=1.0\linewidth]{imgs/result/paper08a_bar_main.pdf} 
	\end{minipage}
	\begin{minipage}{0.33\linewidth}
  		\includegraphics[width=1.0\linewidth]{imgs/result/paper08a_bar_filter.pdf} 
	\end{minipage}
	\begin{minipage}{0.33\linewidth}
  		\includegraphics[width=1.0\linewidth]{imgs/result/paper08a2_bar_main.pdf} 
	\end{minipage}
  \caption{\textbf{Equal-time comparison of different distribution reconstruction techniques, spatial filtering strategies, and neighboring thresholds }on five scenes featuring different light transport effects and complexity. The corresponding images are shown in the supplemental document. 
  } 
  \Description{...}
  \label{fig_val_spatial_bar}
\end{figure*}



In Fig. \ref{fig_result_other}, we compare our approach with MLT \cite{Veach97MLT} and MEMLT \cite{Jakob12}, two typical MCMC approaches. The 
\textsc{Pool} scene is a typical example of challenging paths, and the 
\textsc{Plane} scene contains a normal-mapped conductor with roughness ($\alpha=0.002$).
Both MLT and MEMLT require admissible chains as their seed paths. Simply relying on PT or BDPT to find valid seed paths is inefficient for SDS paths. This results in either energy loss if no seed path is found for a specific region (blue closeups in \textsc{Pool}) or over-bright artifacts where Markov chains get stuck in narrow regions (red closeups in both scenes). 
As our method works in the context of regular Monte Carlo sampling, it is able to produce images free from blotchy artifacts.

\paragraph{Comparison with biased approaches} 


Biased approaches excel at producing noise-free results for complex caustics and hence prevail in the industry.
In Fig. \ref{fig_result_biased}, we conduct an equal-time comparison with Stochastic Progressive Photon Mapping (SPPM) \cite{Hachisuka09SPPM} and Metropolised Bidirectional Estimator (UPSMCMC) \cite{Sik2016RobustLT}.
A slab and a ring are lit by a distant point light encapsulated in a glass sphere.

For a meaningful comparison with SPPM, we decrease the photon lookup radius to the point that the bias is less perceptible. Despite this, the noise level is still higher than ours. It also suffers from visible light leaking at the bottom of the ring. A similar issue occurs for UPSMCMC.
Its MCMC nature also results in an uneven convergence characterized by an overly dark region and visible fireflies.

As an unbiased method, our technique performs independent Monte Carlo estimation without spatial relaxing or reuse, thereby avoiding these problems and producing caustics of high quality with sharp details and low noise.


Fig. \ref{fig_result_mnee} shows a visual comparison with MNEE \cite{Hanika15}. As aforementioned, MNEE cannot find all valid admissible chains in this scene since it relies on deterministic initialization. Generally, this method performs well in simple cases but works inefficiently and tends to be biased (or suffers from extremely high variance if combined with path tracing) in complex scenes with many solutions. The stochastic sampling strategy adopted in our method makes it possible to cover all solutions for a configuration and hence ensures unbiasedness.


\subsection{Validation of building blocks}

In theory, our pipeline supports most feasible spatial neighbor searching and directional density estimation techniques. However, the decision will significantly affect the quality of the sampling. Here, we endeavor to generate such insights by comparing various alternative choices of pipeline components in Fig. \ref{fig_val_spatial} and Fig. \ref{fig_val_spatial_bar}.

\paragraph{Distribution reconstruction.}

We employ STree for approximated spatial nearest neighbor searching when reconstructing the energy distribution, and perform an accurate directional density estimation. 
To evaluate their effectiveness, we compare our method against adaptive quad-tree \cite{Muller17} (\textit{SDTree}) and a variant of our approach with accurate spatial nearest neighbor searching (\textit{KNN}). 

Despite its overall feasibility, \textit{SDTree} introduces 
more noise 
due to its inaccuracy in reconstructing high-frequency distributions.
In contrast, our accurate local density estimation yields more stable convergence with fewer outliers.
Accurate \textit{KNN}
introduces substantial overhead (around 90\% in most scenes) since gathering thousands of nearest samples is costly. On the contrary, querying the STree only requires descending from the root to the leaf node. Consequently, the total overhead of querying and sampling distributions never exceeds 5\% in all our experiments.



\begin{figure}[tbp]
\centering
	\begin{minipage}{1.00\linewidth}
  			\includegraphics[width=1.0\linewidth]{imgs/result/paper02.pdf} % finalized
	\end{minipage}
	\begin{minipage}{1.00\linewidth}
  			\includegraphics[width=1.0\linewidth]{imgs/result/paper02b.pdf} % finalized
	\end{minipage}
	\begin{minipage}{1.00\linewidth}
  			\includegraphics[width=1.0\linewidth]{imgs/result/paper02c.pdf} % finalized
	\end{minipage}
  \caption{\textbf{Equal-time (5 min) comparison} on scenes with varying chain lengths (top), visibility complexity (middle), and emitter radii (bottom). } 
  \Description{...}
  \label{fig_result_complex}
\end{figure}

\paragraph{Spatial filtering.}
We have employed the spatial filtering (\textit{Ours}) to improve robustness. Along with this, we include comparisons with alternative choices: no spatial filtering (\textit{NoFilter}) and \citet{mueller19guiding}'s stochastic filtering (\textit{StochasticFilter}) that randomly jitter the sample's position.
Simply disable filtering produces inferior results with visible artifacts.
Although stochastic filtering has been widely adopted in previous works \cite{Ruppert2020RobustFO, Zhu2021HierarchicalNR}, it also leads to slightly less accuracy and more fireflies.
In contrast, our approach produces results with less noise and fewer outliers with nearly no performance degradation, striking an appropriate balance between overhead and performance. 


\paragraph{Spatial neighboring threshold.}

We also validate our automatic spatial neighboring threshold in Fig. \ref{fig_val_spatial_bar}. Our automatic threshold always predicts a reasonable value and generally outperforms alternative choices, including \citet{mueller19guiding}'s threshold ($4000 \cdot \sqrt{\mathrm{SPP}}$) and variants of our threshold with different coefficients.




\subsection{Impact of scene complexity} 



Our method adapts well to scenes with various intricate structures. 

\paragraph{Chain length.} 
The first row of Fig. \ref{fig_result_complex} conducts a visual comparison against SMS on a series of scenes with an increasing number of transparent slabs. Since SMS neglects energy distributions during specular chain sampling, the variance increases prominently as the number of specular bounces increases. In contrast, by exploiting the continuity of specular manifolds, our method keeps a low variance even in scenes with long specular chains.

\begin{figure}[tbp]
\centering
	\begin{minipage}{1.00\linewidth}
  			\includegraphics[width=0.5\linewidth]{imgs/result/trainplot_lamp.pdf} % finalized
  			\includegraphics[width=0.5\linewidth]{imgs/result/trainplot_slabs.pdf} % finalized
	\end{minipage}
  \caption{\textbf{The impact of training budget and initialization strategies on the rendered image quality}. The number of training samples per pixel is given as the x-axis. Each image is finally generated with 32 spp.}
  \Description{...}
  \label{fig_plot_train}
\end{figure}




\paragraph{Visibility.} 
The second row of Fig. \ref{fig_result_complex} shows a series of scenes with increasing degrees of complex visibility stemming from multiple pillars near a transparent slab. 
SMS hardly samples solutions that pass the visibility test, while we consider visibility by reconstructing distributions from unblocked admissible chains. As a result, our method avoids high variance introduced by occlusions and works well in complex scenes.



\paragraph{Size of light sources.}
In the last row of Fig. \ref{fig_result_complex}, we present a series of scenes with various emitter sizes. 
As the size of the emitter decreases, the frequency of caustics increases. While path-guiding methods work well for large area lights, producing high-frequency caustics can be challenging. Instead, our proposed method addresses this issue by exploring admissible chains through manifold walks, allowing us to handle small area lights and complex caustic patterns effectively.

\subsection{Choice of strategies}



Our pipeline incorporates some design choices. We conduct the following experiments to validate their effectiveness.
 

\paragraph{Training budgets.}
Fig. \ref{fig_plot_train} shows the influence of the training budget on the rendering with the same sample rate. Generally, the variance reduces significantly as the number of training samples increases. This indicates that the training process gradually makes the sampling distribution optimal. 

\paragraph{Initialization.} 
We also compare different initialization strategies in Fig. \ref{fig_plot_train}. Here, \textit{surface} means uniformly sampling $\mathbf{x}_1$ on specular surfaces, \textit{direction} means uniformly choosing $\mbomega_D$ on the hemisphere, and \textit{photon} means reconstructing the initial distribution from 250,000 photons traced by a photon mapper. The comparison shows that initialization using photons leads to better results at the early stage of training. However, after convergence, different initialization strategies perform similarly. This shows that our method is robust to the initial state.


\begin{table*}
  \caption{Rendering statistics of our experiments. }
  \label{tab_stats}
  \begin{tabular}{llcrrrrrrrrr}
    \toprule
    Scene & Figure &  Chain types & \multicolumn{2}{c}{Budget (min.)} & \multicolumn{2}{c}{Sample per pixel} & \multicolumn{3}{c}{Time on specular (min.)} & \#Sub-path \\
    & & (dominant) & Total & Training  & Training & Rendering & Guide & PDF & Total & samples \\
    \midrule
    \textsc{Glass} & Fig. \ref{fig:teaser} & $TT, TTTT, TTTTTT$ & 240.0 & 72.0 & 80 & 195 & 3.592 & 77.886 & 215.328 & 12 519 949  \\
    \textsc{Lamp} & Fig. \ref{fig_result_2} & $T, RT$ & 5.0 & 1.5 & 46 & 116 & 0.233 & 0.388 & 3.377 & 1 347 096 \\
    \textsc{Flower} & Fig. \ref{fig_result_2} & $TT, TTR$ &  5.0 & 1.5 & 16 & 134 & 0.053 & 1.971 & 3.983 & 1 189 876 \\
    \textsc{Double Slabs} & Fig. \ref{fig_result_2} & $TT, TTTT$ & 5.0 & 1.5 & 24 & 59 & 0.096 & 1.433 & 4.127 & 2 066 782 \\ 
    \textsc{Water} & Fig. \ref{fig_result_gow} & $TTTT, TTTTTT$ & 240.0 & 72.0 & 41 & 99 & 2.621 & 223.176 & 236.883 & 1 667 185 \\ % finalized                                                                                                    
  \bottomrule
\end{tabular}
\end{table*}
\subsection{Performance analysis}

In Table \ref{tab_stats}, we report the rendering statistics of several test scenes used in this paper. As seen, for each scene, 50\%-98\% of the time is spent on specular chain sampling. In particular, a small amount of time (no more than 5\% in all the scenes) is spent on guiding (i.e., querying the spatial and directional distributions). In complex scenes, the reciprocal probability estimation has a non-negligible run-time cost since many trials are required. 

\begin{figure}[tbp]
\centering
	\begin{minipage}{1.0\linewidth}
  			\includegraphics[width=1\linewidth]{imgs/result/paper08e_small_slabs.pdf}
	\end{minipage}
  \caption{\ff{The variance of reciprocal probability estimation can be reduced by repeating the process multiple times (4 in this example) and using the average, either in the rendering phase only (R×4) or both training and rendering phases (TR×4). This example also showcases the notable overhead of the estimation process.}
  } 
  \Description{...}
  \label{fig_result_repber}
\end{figure}


Our implementation needs to store the original sample, which could cause relatively heavy storage. Our consideration is twofold. On the one hand, the storage required for each raw sample is only 40 bytes. On the other hand, it is worthy of being done because the local density estimation is more accurate than existing online fitting approaches when faced with near-delta radiance distributions. 



